Global Group Fairness in Federated Learning via Function Tracking

We investigate group fairness regularizers in federated learning, aiming to train a globally fair model in a distributed setting. Ensuring global fairness in distributed training presents unique challenges, as fairness regularizers typically involve probability metrics between distributions across all clients and are not naturally separable by client. To address this, we introduce a function-tracking scheme for the global fairness regularizer based on a Maximum Mean Discrepancy (MMD), which incurs a small communication overhead. This scheme seamlessly integrates into most federated learning algorithms while preserving rigorous convergence guarantees, as demonstrated in the context of FedAvg. Additionally, when enforcing differential privacy, the kernel-based MMD regularization enables straightforward analysis through a change of kernel, leveraging an intuitive interpretation of kernel convolution. Numerical experiments confirm our theoretical insights.

==> figures/flow.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,325); %set diagram left start at 0, and has height of 325

%Shape: Rectangle [id:dp7253182644157948] 
\draw   (30,80) -- (130,80) -- (130,120) -- (30,120) -- cycle ;
%Shape: Rectangle [id:dp6700724260499616] 
\draw   (130,190) -- (230,190) -- (230,230) -- (130,230) -- cycle ;
%Shape: Rectangle [id:dp21289472738312687] 
\draw   (20,20) -- (240,20) -- (240,310) -- (20,310) -- cycle ;
%Straight Lines [id:da9901517786985513] 
\draw    (80,130) -- (80,148) ;
\draw [shift={(80,150)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8260851604842675] 
\draw    (80,54) -- (80,72) ;
\draw [shift={(80,74)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6782276142698876] 
\draw    (180,55) -- (180,178) ;
\draw [shift={(180,180)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9488587271147546] 
\draw    (80,175) -- (80,298) ;
\draw [shift={(80,300)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da967918605948807] 
\draw    (180,238) -- (180,256) ;
\draw [shift={(180,258)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da519870142011752] 
\draw    (180,282) -- (180,300) ;
\draw [shift={(180,302)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da839938127883735] 
\draw    (180,55) -- (101.97,69.63) ;
\draw [shift={(100,70)}, rotate = 349.38] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da1337287593205776] 
\draw    (80,175) -- (158,179.88) ;
\draw [shift={(160,180)}, rotate = 183.58] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (80,32) node [anchor=north ][inner sep=0.75pt]   [align=left] {$\mathcal{Y}^0_{t-1}, \mathcal{Y}^1_{t-1}$};
% Text Node
\draw (180,32) node [anchor=north][inner sep=0.75pt]   [align=left] {$\theta_{t-1}$};
% Text Node
\draw (41,92) node [anchor=north west][inner sep=0.75pt]   [align=left] {Algorithm~\ref{algo:C-tracking}};
% Text Node
\draw (141,205) node [anchor=north west][inner sep=0.75pt]   [align=left] {Algorithm~\ref{algo:theta-update}};
% Text Node
\draw (80,152) node [anchor=north][inner sep=0.75pt]   [align=left] {$\mathcal{Y}^0_{t}, \mathcal{Y}^1_{t}$};
% Text Node
\draw (180,262) node [anchor=north][inner sep=0.75pt]   [align=left] {$\theta_{t}$};


\end{tikzpicture}
